Auto-Encoded Supervision for Perceptual Image Super-Resolution

This work tackles the fidelity objective in the perceptual super-resolution~(SR). Specifically, we address the shortcomings of pixel-level $L_\text{p}$ loss ($\mathcal{L}_\text{pix}$) in the GAN-based SR framework. Since $L_\text{pix}$ is known to have a trade-off relationship against perceptual quality, prior methods often multiply a small scale factor or utilize low-pass filters. However, this work shows that these circumventions fail to address the fundamental factor that induces blurring. Accordingly, we focus on two points: 1) precisely discriminating the subcomponent of $L_\text{pix}$ that contributes to blurring, and 2) only guiding based on the factor that is free from this trade-off relationship. We show that they can be achieved in a surprisingly simple manner, with an Auto-Encoder (AE) pretrained with $L_\text{pix}$. Accordingly, we propose the Auto-Encoded Supervision for Optimal Penalization loss ($L_\text{AESOP}$), a novel loss function that measures distance in the AE space, instead of the raw pixel space. Note that the AE space indicates the space after the decoder, not the bottleneck. By simply substituting $L_\text{pix}$ with $L_\text{AESOP}$, we can provide effective reconstruction guidance without compromising perceptual quality. Designed for simplicity, our method enables easy integration into existing SR frameworks. Experimental results verify that AESOP can lead to favorable results in the perceptual SR task.

==> table/ablation2_table.tex <==
\begin{table}[!h]
\centering
\footnotesize
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\midrule
\multicolumn{1}{c}{} & \multicolumn{1}{|c}{Manga109} & \multicolumn{1}{|c}{General100} & \multicolumn{1}{|c}{Urban100} & \multicolumn{1}{|c}{DIV2K100} & \multicolumn{1}{|c}{BSD100} \\ 
\midrule\midrule
$\text{Ours}$ & \textbf{29.97}/\textbf{.0525} & \textbf{30.48}/\textbf{.0784} & \textbf{25.63}/.1064 & \textbf{29.08}/\textbf{.0977} & \textbf{26.08}/.1515 \\
$\text{(a)}$  & 29.78/.0534 & 30.35/.0789 & 25.55/\textbf{.1054} & 28.97/.0982 & 25.98/\textbf{.1498} \\ % SRResNet
$\text{LDL}$  & 29.62/.0544 & 30.29/.0796 & 25.46/.1084 & 28.82/.0999 & 25.95/.1535 \\
$\text{(b)}$  & 29.55/.0545 & 30.20/.0801 & 25.39/.1090 & 28.75/.1005 & 25.89/.1544 \\ % LP
\midrule
%
%
\end{tabular}
}
\caption{PSNR/LPIPS scores.\textbf{(a)} w/ SRResNet-AE.\textbf{(b)} w/ LP+$\Loss{}_1$.}
\label{tab:ablation2_table}
\end{table}

==> table/ablation_table.tex <==
\begin{table}[!h]
    \centering
    \footnotesize
    \resizebox{0.4\textwidth}{!}{%
    \begin{tabular}{c|ccc|cc}
    \toprule
          & Decoder & Encoder & $\Loss{}^\text{rec}_\text{LR}$ & DISTS~$\downarrow$ & PSNR~$\uparrow$ \\
    \midrule
        LDL & & & & 0.0526 & 28.819 \\
    \midrule
        (a) & \checkmark    &               &               & 0.0521 & 29.060 \\
        (b) & \checkmark    & \checkmark    &               & 0.0526 & \textbf{29.150} \\
        (c) & \checkmark    & \checkmark    & \checkmark    & \textbf{0.0518} & 29.079 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation study on each component of \AAEESOP{}. We report DISTS and PSNR scores of \AAEESOP{}~(128) on DIV2K.}
    \vspace{-5pt}
    \label{tab:ablation_table}
\end{table}

==> table/aepsnr_table.tex <==
\begin{table}[!t]
\vspace{-5pt}
\centering
\setlength{\tabcolsep}{1.5pt}
\footnotesize
\renewcommand{\arraystretch}{0.9} % Adjust row spacing
\begin{tabular}{@{}c|ccccccc@{}}
\midrule
Method & Set14 & Mg109 & Gen100 & Urb100 & DIV2K & B100 & LSDIR \\
\midrule
ESRGAN~\cite{SISR7_ESRGAN}        & 30.280	& 31.165 &	32.663 &	27.198 &	31.668 &	28.991 &	27.636 \\
SPSR~\cite{SPSR}                  & 30.602	& 31.351 &	32.670 &	27.508 &	31.737 &	29.029 &	27.881 \\
LDL~\cite{details_or_artifact}    & 31.180	& 32.608 &	33.823 &	28.488 &	32.597 &	29.595 &	28.625 \\
\rowcolor{gray!20} %
AESOP~(Ours)                      & \textbf{31.341}	& \textbf{32.843} &	\textbf{33.956} &	\textbf{28.529} &	\textbf{32.740} &	\textbf{29.737} &	\textbf{28.812} \\
\hline
\end{tabular}
\vspace{-5pt}
\caption{
AE-PSNR scores for RRDB-backbone (128) methods.
}
\label{tab:maintable}
\end{table}



==> table/lrpsnr_table.tex <==
\begin{table}[!t]
\vspace{-5pt}
\centering
\setlength{\tabcolsep}{1.5pt}
\footnotesize
\renewcommand{\arraystretch}{0.9} % Adjust row spacing
\begin{tabular}{@{}c|ccccccc@{}}
\midrule
Method & Set14 & Mg109 & Gen100 & Urb100 & DIV2K & B100 & LSDIR \\
\midrule
ESRGAN~\cite{SISR7_ESRGAN} & 43.892 & 43.908 & 45.259 & 42.879 & 45.689 & 43.823 & 42.718 \\
SPSR~\cite{SPSR}   & 43.835 & 44.359 & 44.656 & 42.666 & 44.717 & 42.719 & 42.364 \\
LDL~\cite{details_or_artifact}    & 46.497 & 47.603 & 48.184 & 45.975 & 47.793 & 45.307 & 45.295 \\
\rowcolor{gray!20} %
AESOP~(Ours)  & \textbf{46.625} & \textbf{48.188} & \textbf{48.653} & \textbf{46.280} & \textbf{48.272} & \textbf{45.837} & \textbf{45.571} \\
\hline
\end{tabular}
\vspace{-5pt}
\caption{
LR-PSNR scores for RRDB-backbone (128) methods.
}
\label{tab:maintable}
\end{table}



==> table/main_table2.tex <==
\begin{table*}[!t]
\vspace{-5pt}
\centering
\renewcommand{\arraystretch}{0.9} % Adjust row spacing
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cl|cccc|cc|ccccc@{}}
\toprule
 & Backbone & \multicolumn{6}{c|}{RRDB} & \multicolumn{5}{c}{SwinIR} \\ 
\midrule\midrule
\multicolumn{1}{c}{Metrics} &
  \multicolumn{1}{l|}{Benchmark} &
  ESRGAN &
  SPSR &
  LDL &
  \multicolumn{1}{c|}{AESOP} &
  \multicolumn{1}{c}{CALGAN} &
  \multicolumn{1}{c|}{AESOP} &
  \multicolumn{1}{c}{+GAN} &
  LDL &
  CALGAN &
  AESOP &
  AESOP^* \\ 
\midrule
\multicolumn{2}{l|}{\makecell{Patch size (Training)}} & 128 & 128 & 128 & 128 & 256 & 256 & 256 & 256 & 256 & 256 & 256\\
\midrule
\multirow{7}{*}{LPIPS~$\downarrow$} & Set14                   & 0.1241  & 0.1207  & 0.1132  & \textbf{0.1067}  & -      & 0.1053  & 0.1160 & 0.1091  & -     & 0.1027  & \textbf{0.1023} \\
                       & Manga109                             & 0.0649  & 0.0672  & 0.0544  & \textbf{0.0525}  & -      & 0.0494  & 0.0542 & 0.0469  & -     & 0.0461  & \textbf{0.0440} \\
                       & General100                           & 0.0879  & 0.0862  & 0.0796  & \textbf{0.0784}  & 0.077  & \textbf{0.0734}  & 0.0796 & 0.0740  & 0.074 & \textbf{0.0710}   & 0.0717 \\
                       & Urban100                             & 0.1229  & 0.1184  & 0.1084  & \textbf{0.1064}  & 0.108  & \textbf{0.1033}  & 0.1077 & 0.1021  & 0.098 & \textbf{0.0945}  & 0.0961 \\
                       & DIV2K-val                             & 0.1154  & 0.1099  & 0.0999  & \textbf{0.0977}  & \textbf{0.091}  & 0.0936  & 0.1038 & 0.0944  & \textbf{0.087} & 0.0893  & 0.0909 \\
                       & BSD100$^\dagger$                     & 0.1616  & 0.1609  & 0.1535  & \textbf{0.1515}  & 0.151  & \textbf{0.1443}  & -      & 0.1572  & 0.147 & \textbf{0.1385}  & 0.1441 \\
                       & LSDIR$^\dagger$                      & 0.1378  & 0.1312  & 0.1180  & \textbf{0.1152}  & -      & 0.1123  & -      & 0.1132  & -     & \textbf{0.1071}  & 0.1094 \\ 
                       \midrule
\multirow{7}{*}{DISTS~$\downarrow$} & Set14                     & 0.0951  & 0.0920  & 0.0866  & \textbf{0.0852}  & -      & 0.0825  & 0.0930 & 0.0869  & -     & 0.0819  & \textbf{0.0809} \\
                       & Manga109                             & 0.0471  & 0.0463  & \textbf{0.0355}  & 0.0360   & -      & 0.0356  & 0.0365 & \textbf{0.0315}  & -     & 0.0328  & 0.0327 \\
                       & General100                           & 0.0874  & 0.0884  & 0.0801  & \textbf{0.0798}  & 0.083  & \textbf{0.0773}  & 0.0835 & 0.0794  & 0.081 & \textbf{0.0762}  & 0.0768 \\
                       & Urban100                             & 0.0880  & 0.0849  & \textbf{0.0793}  & \textbf{0.0793}  & 0.082  & \textbf{0.0768}  & 0.0835 & 0.0800  & 0.083 & \textbf{0.0742}  & 0.0751 \\
                       & DIV2K-val                             & 0.0593  & 0.0546  & 0.0526  & \textbf{0.0518}  & 0.049  & \textbf{0.0484}  & 0.0531 & 0.0507  & 0.048 & \textbf{0.0459}  & 0.0469 \\
                       & BSD100$^\dagger$                     & 0.1165  & 0.1176  & 0.1163  & \textbf{0.1117}  & 0.118  & \textbf{0.1089}  & -      & 0.1185  & 0.128 & \textbf{0.1072}  & 0.1078 \\
                       & LSDIR$^\dagger$                      & 0.0764  & 0.0699  & 0.0650  & \textbf{0.0641}  & -      & 0.0612  & -      & 0.0650  & -     & \textbf{0.0591}  & 0.0601 \\ 
                       \midrule
\multirow{7}{*}{PSNR~$\uparrow$}  & Set14                       & 26.594  & 26.860  & 27.228  & \textbf{27.361}  & -      & 27.246  & 27.282 & 27.526  & -     & 27.421 & \textbf{27.822} \\
                       & Manga109                             & 28.413  & 28.561  & 29.620  & \textbf{29.973}  & -      & 29.747  & 29.345 & 30.143  & -     & 30.061 & \textbf{30.453} \\
                       & General100                           & 29.425  & 29.424  & 30.289  & \textbf{30.482}  & 30.182 & \textbf{30.251}  & 30.104 & 30.441  & -     & 30.401 & \textbf{30.752} \\
                       & Urban100                             & 24.365  & 24.804  & 25.459  & \textbf{25.630}  & 25.290 & \textbf{25.541}  & 25.736 & 26.231  & -     & 26.148 & \textbf{26.398} \\
                       & DIV2K-val                             & 28.175  & 28.182  & 28.819  & \textbf{29.079}  & 28.863 & \textbf{28.910}  & 28.784 & 29.117  & -     & 29.137 & \textbf{29.543} \\
                       & BSD100$^\dagger$                     & 25.313  & 25.501  & 25.954  & \textbf{26.080}  & \textbf{25.925} & 25.904  & -      & 26.216  & -     & 25.930 & \textbf{26.405} \\
                       & LSDIR$^\dagger$                      & 23.882  & 24.232  & 24.663  & \textbf{24.933}  & -      & 24.845  & -      & 25.129  & -     & 25.038 & \textbf{25.419} \\ 
                       \midrule

\multirow{7}{*}{SSIM~$\uparrow$}  & Set14                       & 0.7144  & 0.7254  & 0.7358  & \textbf{0.7402}  & -      & 0.7371  & 0.7407 & 0.7478  & -     & 0.7438  & \textbf{0.7578} \\
                       & Manga109                             & 0.8595  & 0.8590  & 0.8734  & \textbf{0.8827}  & -      & 0.8802  & 0.8796 & 0.8880   & -     & 0.8880   & \textbf{0.8949}  \\
                       & General100                           & 0.8095  & 0.8091  & 0.8280  & \textbf{0.8335}  & 0.825  & \textbf{0.8269}  & 0.8305 & 0.8347  & -     & 0.8328  & \textbf{0.8415} \\
                       & Urban100                             & 0.7341  & 0.7474  & 0.7661  & \textbf{0.7724}  & 0.763  & \textbf{0.7697}  & 0.7786 & 0.7918  & -     & 0.7884  & \textbf{0.7947} \\
                       & DIV2K-val                             & 0.7759  & 0.7720  & 0.7897  & \textbf{0.7978}  & 0.790  & \textbf{0.7951}  & 0.7911 & 0.8011  & -     & 0.8023  & \textbf{0.8121} \\
                       & BSD100$^\dagger$                     & 0.6527  & 0.6596  & 0.6813  & \textbf{0.6841}  & 0.676  & \textbf{0.6783}  & -      & 0.6923  & -     & 0.6813  & \textbf{0.6982} \\
                       & LSDIR$^\dagger$                      & 0.6866  & 0.6966  & 0.7117  & \textbf{0.7220}  & -      & 0.7202  & -      & 0.7316  & -     & 0.7289  & \textbf{0.7397} \\  
                       \midrule
\multirow{7}{*}{PSNR_{LR}~$\uparrow$}  & Set14$^\dagger$                & 43.892  & 43.835  & 46.497  & \textbf{46.625}  & -      & 46.148  & -      & 46.899  & -     & 46.534 & \textbf{48.245} \\
                       & Manga109$^\dagger$                             & 43.908  & 44.359  & 47.603  & \textbf{48.188}  & -      & 47.831  & -      & 49.135  & -     & 48.794 & \textbf{50.042} \\
                       & General100$^\dagger$                           & 45.259  & 44.656  & 48.184  & \textbf{48.653}  & -      & 47.949  & -      & 48.663  & -     & 48.101 & \textbf{49.733} \\
                       & Urban100$^\dagger$                             & 42.879  & 42.666  & 45.975  & \textbf{46.280}  & -      & 45.979  & -      & 47.404  & -     & 47.321 & \textbf{48.564} \\
                       & DIV2K-val$^\dagger$                             & 45.689  & 44.717  & 47.793  & \textbf{48.272}  & -      & 47.487  & -      & 48.084  & -     & 47.924 & \textbf{49.856} \\
                       & BSD100$^\dagger$                     & 43.823  & 42.719  & 45.307  & \textbf{45.837}  & -      & 45.072  & -      & 45.494  & -     & 45.036 & \textbf{47.578} \\
                       & LSDIR$^\dagger$                      & 42.718  & 42.364  & 45.295  & \textbf{45.571}  & -      & 44.998  & -      & 45.731  & -     & 45.604 & \textbf{47.476} \\ 
                       \hline\hline
\end{tabular}%
}
\caption{
Quantitative results of the proposed method~(\AAEESOP{}) against baseline methods. The best results of each group are highlighted in \textbf{bold}. Scores that are not reported in the official papers are re-evaluated by provided weights, indicated as $\dagger$. \AAEESOP{}$^*$ indicates only training 200K iterations, whereas a fully trained model takes 300K steps. $\uparrow$ means higher is better, $\downarrow$ means lower is better.
}
\vspace{-10pt}
\label{tab:maintable}
\end{table*}


